Optimal Transport Metric Learning for Feature Alignment in Partially Supervised Segmentation

Multi-organ segmentation is often challenged by partially annotated datasets and domain shifts across different imaging sources. To address these limitations, we propose a two-stage learning framework that efficiently leverages partial supervision. In the first stage, the model learns from available annotations to produce accurate segmentations of annotated organs, establishing robust feature representations. In the second stage, we introduce learnable organ prototypes and a Sinkhorn-triplet loss to enforce organ-wise feature consistency across datasets. This encourages latent embeddings of the same organ to remain close, while increasing separation between different organs, even when annotations are missing. Our approach achieves performance comparable to state-of-the-art methods on the BTCV dataset, while remaining computationally efficient. By explicitly aligning feature distributions rather than relying solely on pseudo-labels, the framework effectively mitigates domain shift, making it particularly suitable for medical image segmentation tasks with limited annotation resources.

==> newsv-mult/author/references.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
%\biblstarthook{


\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
\bibitem{gonzalez2018multi}
González, G., Washko, G.R., San José Estépar, R.:
Multi-structure segmentation from partially labeled datasets: application to body composition measurements on CT scans.
In: International Workshop on Reconstruction and Analysis of Moving Body Organs, pp. 215--224. Springer (2018)

\bibitem{schutera2022methods}
Schutera, M., Rettenberger, L., Pylatiuk, C., Reischl, M.:
Methods for the frugal labeler: multi-class semantic segmentation on heterogeneous labels.
Plos One, 17(2), e0263656 (2022)

\bibitem{zhang2021dodnet}
Zhang, J., Xie, Y., Xia, Y., Shen, C.:
Dodnet: learning to segment multi-organ and tumors from multiple partially labeled datasets.
In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 1195--1204 (2021)

\bibitem{deng2021omni}
Deng, R., Liu, Q., Cui, C., Asad, Z., Yang, H., Huo, Y.:
Omni-Seg: a single dynamic network for multi-label renal pathology image segmentation using partially labeled data.
arXiv:2112.12665 (2021)

\bibitem{liu2024cosst}
Liu, H., Xu, Z., Gao, R., Li, H., Wang, J., Chabin, G., Oguz, I., Grbic, S.:
Cosst: multi-organ segmentation with partially labeled datasets using comprehensive supervisions and self-training.
IEEE Transactions on Medical Imaging, 43(5), 1995--2009. IEEE (2024)

\bibitem{liu2024many}
Liu, Q., Zeng, H., Sun, Z., Li, X., Zhao, G., Liang, Y.:
Many birds, one stone: medical image segmentation with multiple partially labeled datasets.
Pattern Recognition, 155, 110636. Elsevier (2024)

\bibitem{gorade2025otcxr}
Gorade, V., Sing, A., Mishra, D.:
OTCXR: rethinking self-supervised alignment using optimal transport for chest X-ray analysis.
In: 2025 IEEE/CVF Winter Conference on Applications of Computer Vision (WACV), pp. 7143--7152. IEEE (2025)

\bibitem{arjovsky2017wasserstein}
Arjovsky, M., Chintala, S., Bottou, L.:
Wasserstein generative adversarial networks.
In: International Conference on Machine Learning, pp. 214--223. PMLR (2017)

\bibitem{feydy2019interpolating}
Feydy, J., Séjourné, T., Vialard, F.-X., Amari, S., Trouvé, A., Peyré, G.:
Interpolating between optimal transport and MMD using Sinkhorn divergences.
In: The 22nd International Conference on Artificial Intelligence and Statistics, pp. 2681--2690. PMLR (2019)

\bibitem{shi2021marginal}
Shi, G., Xiao, L., Chen, Y., Zhou, S.K.:
Marginal loss and exclusion loss for partially supervised multi-organ segmentation.
Medical Image Analysis, 70, 101979. Elsevier (2021)

\bibitem{ding2023cross}
Ding, R., Zhou, Y., Xu, J., Xie, Y., Liang, Q., Ren, H., Wang, Y., Chen, Y., Wang, L., Huang, M.:
Cross-hospital sepsis early detection via semi-supervised optimal transport with self-paced ensemble.
IEEE Journal of Biomedical and Health Informatics, 27(6), 3049--3060. IEEE (2023)

\bibitem{janati2019wasserstein}
Janati, H., Cuturi, M., Gramfort, A.:
Wasserstein regularization for sparse multi-task regression.
In: The 22nd International Conference on Artificial Intelligence and Statistics, pp. 1407--1416. PMLR (2019)

\bibitem{sarlin2020superglue}
Sarlin, P.-E., DeTone, D., Malisiewicz, T., Rabinovich, A.:
SuperGlue: learning feature matching with graph neural networks.
In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 4938--4947 (2020)

\bibitem{demir2023topology}
Demir, A., Massaad, E., Kiziltan, B.:
Topology-aware focal loss for 3D image segmentation.
In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pp. 580--589 (2023)

\bibitem{antonelli2022msd}
Antonelli, M., Reinke, A., Bakas, S., Farahani, K., Kopp-Schneider, A., Landman, B.A., Litjens, G., Menze, B., Ronneberger, O., Summers, R.M., et al.:
The medical segmentation decathlon.
Nature Communications, 13(1), 4128 (2022)

\bibitem{heller2021kits19}
Heller, N., Isensee, F., Maier-Hein, K.H., Hou, X., Xie, C., Li, F., Nan, Y., Mu, G., Lin, Z., Han, M., et al.:
The state of the art in kidney and kidney tumor segmentation: results of the KiTS19 challenge.
Medical Image Analysis, 67, 101821. Elsevier (2021)

\bibitem{landman2015btcv}
Landman, B., Xu, Z., Igelsias, J., Styner, M., Langerak, T., Klein, A.:
MICCAI multi-atlas labeling beyond the cranial vault—workshop and challenge.
In: Proc. MICCAI Multi-Atlas Labeling Beyond Cranial Vault—Workshop Challenge, vol. 5, p. 12 (2015)

\bibitem{isensee2021nnu}
Isensee, F., Jaeger, P.F., Kohl, S.A.A., Petersen, J., Maier-Hein, K.H.:
nnU-Net: a self-configuring method for deep learning-based biomedical image segmentation.
Nature Methods, 18(2), 203--211 (2021)

\bibitem{bilic2023liver}
Bilic, P., Christ, P., Li, H.B., Vorontsov, E., Ben-Cohen, A., Kaissis, G., Szeskin, A., Jacobs, C., Mamani, G.E., Chartrand, G., et al.:
The liver tumor segmentation benchmark (LiTS).
Medical Image Analysis, 84, 102680. Elsevier (2023)

\bibitem{dou2022optimaltriplet}
Dou, J.X., Luo, L., Yang, R.M.:
An optimal transport approach to deep metric learning (student abstract).
In: Proceedings of the AAAI Conference on Artificial Intelligence, 36(11), 12935--12936 (2022)

\bibitem{varior2016siamese}
Varior, R.R., Shuai, B., Lu, J., Xu, D., Wang, G.:
A siamese long short-term memory architecture for human re-identification.
In: European Conference on Computer Vision, pp. 135--153. Springer (2016)

\bibitem{schroff2015facenet}
Schroff, F., Kalenichenko, D., Philbin, J.:
FaceNet: a unified embedding for face recognition and clustering.
In: Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition, pp. 815--823 (2015)

\bibitem{vinyals2016matching}
Vinyals, O., Blundell, C., Lillicrap, T., Wierstra, D., et al.:
Matching networks for one-shot learning.
Advances in Neural Information Processing Systems, 29 (2016)

\bibitem{hadsell2006contrastive}
Hadsell, R., Chopra, S., LeCun, Y.:
Dimensionality reduction by learning an invariant mapping.
In: 2006 IEEE Conference on Computer Vision and Pattern Recognition (CVPR'06), vol. 2, pp. 1735--1742. IEEE (2006)

\bibitem{kulis2011dpmeans}
Kulis, B., Jordan, M.I.:
Revisiting k-means: new algorithms via Bayesian nonparametrics.
arXiv:1111.0352 (2011)

\bibitem{fang2020tal}
Fang, X., Yan, P.:
Multi-organ segmentation over partially labeled datasets with multi-scale feature abstraction.
IEEE Transactions on Medical Imaging, 39(11), 3619--3629. IEEE (2020)

\bibitem{liu2022universal}
Liu, P., Deng, Y., Wang, C., Hui, Y., Li, Q., Li, J., Luo, S., Sun, M., Quan, Q., Yang, S., et al.:
Universal segmentation of 33 anatomies.
arXiv:2203.02098 (2022)

\bibitem{huang2020cotraining}
Huang, R., Zheng, Y., Hu, Z., Zhang, S., Li, H.:
Multi-organ segmentation via co-training weight-averaged models from few-organ datasets.
In: International Conference on Medical Image Computing and Computer-Assisted Intervention, pp. 146--155. Springer (2020)

\bibitem{jiang2025labeledtounlabeled}
Jiang, X., Zhang, D., Li, X., Liu, K., Cheng, K.-T., Yang, X.:
Labeled-to-unlabeled distribution alignment for partially supervised multi-organ medical image segmentation.
Medical Image Analysis, 99, 103333. Elsevier (2025)

% Contribution 
% \bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
% %
% % Online Document
% \bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Monograph
% \bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
% %
% % Journal article
% \bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
% %
% % Journal article by DOI
% \bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
% %
% %\bigskip

% % Use the following (APS) syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Mathematics, Physics, Statistics, Computer Science"
% %
% % Online Document
% \bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Monograph
% \bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
% %
% % Journal article
% \bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
% %
% % Journal article by DOI
% \bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
% %
% % Contribution 
% \bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593

% %
% % Use the following syntax and markup for your references if 
% % the subject of your book is from the field 
% % "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
% %
% %
% % Contribution 
% \bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
% %
% % Online Document
% \bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
% \url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
% %
% % Journal article by DOI
% \bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
% %
% % Journal article
% \bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
% %
% % Monograph
% \bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
% %
\end{thebibliography}

